Astar: Learning to Propose Evolution Directions for Self-Evolving Industrial AI Systems

Modern AI systems advance through continuous iteration: a loop of proposing evolution directions, implementing code, training, and evaluation. While the latter three stages are increasingly automated, the starting point --- proposing effective evolution directions --- remains a critical bottleneck that still relies heavily on senior experts. In this work, we explore whether AI can take over this role. We find that general-purpose LLMs, even the advanced GPT-5.5, offer only generic and misaligned suggestions: the required expertise is accumulated through experience rather than explicitly codified, and thus hard to inject directly. To this end, we propose Astar, a training-based approach that learns a specialized evolution-guiding model from the abundant iteration histories of industrial systems. Realizing this idea, however, raises four challenges: sparse supervision, noisy data, a vast direction space, and prohibitively expensive verification. We address them along two fronts. On the data side, we design a pipeline that turns noisy historical commits into a large, clean evolutionary corpus via pairwise sample expansion and noise filtering. On the model side, we train the model through mid-training, SFT, and RL, guiding evolution direction generation with hierarchical hints and using the reward model in RL as a fast surrogate evaluator. Astar has been deployed in Alibaba's Lazada advertising system for evolution direction proposal. Astar-8B achieves a single-proposal success rate of 0.6786 in real-execution evaluation, far exceeding human experts (0.3229) and the strongest general-purpose LLM (0.3071). More importantly, Astar closes the loop and enables fully automatic iteration: it guided 20 consecutive iterations over two weeks, improving offline Hitrate@200 by 23.6%, while an online A/B test yielded relative lifts of 4.86% in GMV and 1.82% in advertising revenue.

==> sections/3_data.tex <==
\section{Decision Corpus Construction}
\label{sec:data}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/Figure_data.pdf}
    \caption{The decision corpus construction pipeline.}
    \label{fig:data_pipeline}
\end{figure}
The quality of Astar is decided here: the corpus is what converts a target system's raw iteration history into learnable decisions. The raw material is millions of experiment records accumulated over one year by recommendation-domain teams~\cite{covington2016youtube,cheng2016widedeep,zhou2018din,guo2017deepfm,wang2017dcn,naumov2019dlrm,lwgr,reg4rec}, each a complete snapshot of one training task (engineering code, the per-step loss log, and experiment metadata; full schema in Appendix~\ref{app:data}). Two of our three challenges live in this raw material. The signal is scarce (C3): most commits are not comparable, so single-commit labels waste the history. The signal is also buried (C2): most edits are noise, and the same intent takes different code forms across repositories. The pipeline below is designed directly against these two problems, in four stages: pairing, noise filtering, semantic extraction, and label normalization.

\subsection{Data Source and Pairing}
The unit Astar learns from is not one snapshot but a change and the effect it induces, which forces the basic training example to be a comparison between two versions. The scarcity in C3 comes from insisting that the two versions be adjacent commits: clean, comparable neighbors are rare. Our way out is an observation about the data itself. Every experiment independently records its full loss-convergence curve, so the loss curve is an \emph{absolute} quality measure, and the relative quality of any two runs follows from comparing their curves regardless of whether they are temporally adjacent. This removes the adjacency requirement entirely. We group experiments by $(\text{user\_id}, \text{git\_repo})$, which is one engineer's iteration trajectory on one system, and within each group form all $\binom{n}{2}$ ordered pairs $(prev, cur)$ instead of only the $n-1$ neighbors. The code difference of a pair is the decision content and its loss change is the outcome label, produced automatically with no human involvement. Full pairwise combination is what turns a fixed, scarce set of records into a corpus orders of magnitude larger, which is our primary answer to C3.

\subsection{Noise Filtering}
Expanding to all pairs sharpens C2: the more pairs we form, the more of them are pseudo-changes such as path edits, log or formatting tweaks, resource reconfigurations, and debugging statements, which produce a diff but carry no decision. Left in, they would teach the model irrelevant patterns and drown the real optimization intent. Rather than one blunt heuristic, we use a three-layer filter, because noise hides at three different granularities and each layer removes what the previous one cannot see.

\paragraph{Configuration keys.}
The first layer targets changes that touch only configuration files, where an identical-looking key edit can be either a real decision (\texttt{learning\_rate}, \texttt{batch\_size}, \texttt{optimizer}, \texttt{model\_name}) or a pure environment switch (\texttt{output\_dir}, \texttt{job\_name}, data-table paths, platform resources). We classify each changed key with a whitelist rule that marks as noise only keys with clearly no training significance and conservatively keeps everything else, including unrecognized keys; a file whose changed keys are all noise is a pseudo-change (full key lists in Appendix~\ref{app:data}).

\paragraph{AST normalization.}
The second layer targets \texttt{.py} edits that change text but not behavior, since a text diff cannot separate a real logical change from added prints, edited docstrings, or reordered imports~\cite{allamanis2018survey,alon2019code2vec,feng2020codebert}. We normalize each file through its abstract syntax tree, stripping prints and docstrings and sorting imports, and treat the change as a pseudo-change when $prev$ and $cur$ normalize to identical code.

\paragraph{Entry reachability.}
The third layer catches noise no single-file check can, namely edits to code the experiment never runs: a repository may keep several model versions while only one is live. Starting from the entry scripts declared in shell and configuration files, we traverse the import chain to find every file the experiment actually reaches and drop changes to unreachable dead code. The same analysis resolves configuration routing: when a config field points to \texttt{model\_v3.py} in $prev$ and \texttt{model\_v4.py} in $cur$, it pairs the two model files so semantic analysis compares the code that truly changed rather than a routing pointer (details in Appendix~\ref{app:data}).

\subsection{Insight Extraction}
Filtering leaves real logical changes, but training on the diffs themselves is the wrong target, and this is the most consequential design decision in the pipeline. The same intent, say adding a feature-crossing layer, maps to very different edits across projects, so a model trained on diffs would memorize a codebase's local style rather than a transferable regularity. The deeper point is a division of labor. Reading code and summarizing what it does is exactly what general-purpose LLMs already do well from massive public corpora~\cite{chen2021codex,li2023starcoder,roziere2023codellama,nijkamp2023codegen,guo2024deepseekcoder,hui2024qwen25coder,jimenez2024swebench,li2022alphacode,bavarian2022fim}; what no public corpus contains is whether a given kind of change actually helped a specific system in real training. We therefore delegate code understanding to a general LLM and spend all of our scarce domain data on the part only iteration history can teach: the mapping from intent to real effect. Concretely, we rewrite each diff into a natural-language \emph{insight} of its optimization intent, which also collapses heterogeneous implementations into a finite set of intent clusters and sharply improves sample efficiency under limited data. This abstraction is what current scale rewards; with much larger data, modeling directly from code should have a higher ceiling, which we leave to future work.

Two design details make the insight learnable rather than free-form text. First, generation runs under a fixed Skill definition that forbids any mention of metrics or effect, so an insight encodes intent only and never leaks the outcome it will be trained to predict. Second, each insight carries a three-level label that moves from a major technical direction tag, to a targeted module tag, to a specific change tag. The label supplies grouping the model would otherwise have to rediscover from raw text, and doubles as a quality gate: an insight that matches no legal label in the closed vocabulary is usually too vague or off-scope (vocabulary in Appendix~\ref{app:data}).

\subsection{Environment Features}
An insight states intent, but the same intent can help or hurt depending on where it is applied, so a decision needs its context. Each sample therefore carries two extra components. The base-code description is an LLM-written overview of the $prev$ codebase (model type, core modules, training strategy), giving the prior a decision depends on. The data feature is a structured statistic of the training data (business domain, sample and user counts, sequence-length distribution, cold-start ratio, feature dimensionality) read from the experiment metadata. Together with the labeled insight, these form the complete decision context the model learns from.

\section{Mid-Training}
The staged recipe that answers C3 begins here. Post-training will use only the scarce high-quality pairs, but the surrounding corpus is far larger, and mid-training is how we put that larger corpus to work before decisions are ever learned. Its goal is not to decide which change is better but to transfer a capability: the structured semantic components above are produced by a large LLM, and a small base model has never seen this organization, so it first has to learn the mapping from raw code changes to structured descriptions. A small model cannot acquire this mapping from the limited high-quality set alone, which is precisely why a separate mid-training stage exists.

We therefore run next-token prediction over the full structured corpus~\cite{brown2020gpt3}, keeping every pipeline sample without quality filtering, including negative-outcome changes: understanding and expression are the objective here, and negative samples carry equally well-formed insights, labels, and features, so the full set maximizes exposure to edit patterns and description styles. Each sample is serialized into one sequence (data feature, base insight, three-level labels, diff insight; template in Appendix~\ref{app:impl}) with the loss applied over all tokens, so the model learns both field content and the dependencies among fields. Because every label and feature term comes from real domain records, the model also absorbs domain semantics that generic pretraining lacks. We instantiate mid-training on Qwen-3 base models~\cite{qwen3} at 0.6B, 4B, and 8B. The result is a model that emits correctly formatted fields from a given context and holds stable representations of common optimization patterns, which is the initialization post-training needs.


==> sections/3_data_v1.tex <==
\section{Decision Corpus Construction}
\label{sec:data}
\begin{figure}[htbp]
    \centering
    % \includegraphics[width=1.0\textwidth]{figures/data_pipeline_v1.pdf}
    \includegraphics[width=1.0\textwidth]{figures/data_pipeline_v2.pdf}
    \caption{The decision corpus construction pipeline.}
    \label{fig:data_pipeline}
\end{figure}
To enable Astar to learn effective model evolution strategies from historical developer trajectories, we construct a specialized decision corpus based on git commits and experimental logs. 
However, directly utilizing these raw records presents two critical challenges:
(1) \textit{Data sparsity}, where meaningful algorithmic updates between strictly adjacent commits are exceedingly rare, leading to a severe lack of dense supervision signals;
(2) \textit{Data noise}, where raw code diffs are highly noisy, frequently entangling core algorithmic changes with trivial engineering modifications or tweaks lacking explicit evolutionary intent. 
In this section, we introduce a comprehensive data processing pipeline designed to overcome these hurdles, transforming raw historical logs into a high-quality, structured corpus of state-to-action evolutionary pairs.
The pipeline for decision corpus construction is shown in Figure~\ref{fig:data_pipeline}.

\subsection{Data Expansion}
A primary challenge in leveraging historical commit logs for model evolution is \textit{data sparsity}. 
For a given developer within a specific repository (\texttt{git\_repo}), the historical commits form a chronological sequence $\{C_1, C_2, \dots, C_n\}$.
In real-world industrial settings, relying exclusively on strictly adjacent code commits (i.e., $C_t \rightarrow C_{t+1}$) yields insufficient training data and often captures incomplete micro-edits rather than meaningful evolutionary steps. 
To overcome this limitation, we propose a pairwise data expansion strategy. 
Instead of only extracting consecutive pairs, we generate all possible combinations by pairing any two commits $(C_i, C_j)$ where $i < j$, forming $(C_{prev}, C_{cur})$ training samples. 
This combinatorial approach transforms a sparse commit sequence into a dense dataset. Beyond simply amplifying the sample size, it enables Astar to learn evolutionary trajectories across varying temporal distances, capturing both short-term tweaks and long-term algorithmic leaps.

\subsection{Data Denoising}
Beyond data sparsity, historical commit logs suffer from severe \textit{noise}. Real-world repository modifications frequently mix core algorithmic evolutions with trivial engineering configurations, and many commits lack explicit evolutionary intentions. To extract high-quality supervision signals, we implement a two-stage denoising pipeline comprising rule-based Execution Logic Filtering and LLM-based Evolution Intent Filtering.

\subsubsection{Execution Logic Filtering}
This initial stage aims to isolate modifications that genuinely alter the algorithmic behavior of the model. By applying static code analysis and predefined rules, we systematically strip away non-algorithmic engineering adjustments to obtain a purified execution-level code diff.

\paragraph{Reachability Analysis.} 
To ensure the extracted modifications are actually invoked during the model's lifecycle, we construct a call-graph for the modified codebase. Any changes residing in uncalled functions or unreachable branches are identified as dead code and discarded, ultimately resulting in a strictly pure codebase.


\paragraph{Syntax Normalization.} 
We parse the code files into Abstract Syntax Trees (ASTs) to eliminate syntax-level noise that does not affect model execution. This process automatically detects and removes trivial modifications, including debugging statements (e.g., \texttt{print}, \texttt{assert}), code comments, formatting adjustments, and \texttt{import} sequence reordering.

\paragraph{Configuration Whitelisting.} 
To distinguish between environment setups and algorithmic hyperparameters, we filter modified variables based on a predefined parameter whitelist. Modifications to engineering variables (e.g., \texttt{output\_dir}, \texttt{gpu\_count}, \texttt{job\_name}) are discarded, while changes to core algorithmic parameters (e.g., \texttt{learning\_rate}, \texttt{optimizer}, \texttt{model\_name}) are preserved.

\subsubsection{Evolution Intent Filtering}
Even after obtaining pure code diffs, certain commits may still lack a purposeful model evolution intent. To address this, we leverage Large Language Models (LLMs) to map raw code modifications into explicit evolutionary semantics. Diffs that fail to map to valid evolution intents are regarded as noise and discarded, ensuring that heterogeneous code changes converge into a unified evolution intent space.

\paragraph{Taxonomy Alignment via Hierarchical Hints.} 
We prompt the LLM to classify the pure diff into a predefined three-level taxonomy tree (\textit{L1 Main Direction} $\rightarrow$ \textit{L2 Target Module} $\rightarrow$ \textit{L3 Specific Action}), forming structured \textit{Hierarchical Hints}. These hierarchical hints effectively filter out irrelevant modifications while providing Astar with dense, multi-granular supervision signals during training, and serving as structured priors to guide exploration of evolution directions during inference.

\paragraph{Fine-Grained Elaboration via Diff Insight.} 
Complementing the structured taxonomy, we task the LLM with generating a \textit{Diff Insight}, which is a concise textual explanation detailing the exact code modifications. This insight captures nuanced algorithmic tweaks that the predefined taxonomy might miss, enriching the dataset with a fine-grained semantic description of the evolution intent.

\subsection{Context Construction}
To predict the optimal evolution direction, Astar must understand the system's state prior to modification. For each $(prev, cur)$ pair, we construct a comprehensive system context comprising two key components: \textit{Data Features}, which provide structured statistics of the experimental dataset (e.g., business domain, sample volume, feature dimensions) as a quantitative baseline; and a \textit{Base Insight}, an LLM-generated natural language overview of the \textit{prev} codebase summarizing the existing model architecture, core modules, and training strategies.

By pairing this state context with the denoised evolutionary signals, we formulate the final training corpus. Each instance structurally maps the initial system state to the intended evolutionary action in the format shown in Figure~\ref{fig:data_format}.
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/data_format.pdf}
    \caption{The format of the data.}
    \label{fig:data_format}
\end{figure}
% \begin{Verbatim}[fontsize=\small]
% [Data Feature] <structured statistics of the training data>
% [Base Insight] <natural language overview of the previous codebase>
% ---
% [Level-1] <first-level evolution direction>
% [Level-2] <second-level target module>
% [Level-3] <third-level specific action>
% [Diff Insight] <description of the specific change intent>
% \end{Verbatim}

==> sections/3_data_v2.tex <==
\section{Decision Corpus Construction}
\label{sec:data}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/data_pipeline_v2.pdf}
    \caption{The decision corpus construction pipeline.}
    \label{fig:data_pipeline}
\end{figure}

To enable Astar to learn effective model evolution strategies from historical developer trajectories, we construct a specialized decision corpus based on git commits and experimental logs. 
However, directly utilizing these raw records presents two critical challenges: 
(1) \textit{Data sparsity}, where meaningful algorithmic updates between strictly adjacent experiments are exceedingly rare; 
and (2) \textit{Data noise}, where raw code modifications frequently entangle core algorithmic changes with trivial engineering tweaks, and some updates lack explicit evolutionary intent.
In this section, we introduce a comprehensive data processing pipeline, shown in Figure~\ref{fig:data_pipeline}, transforming raw historical logs into a high-quality, structured corpus of state-to-action evolutionary pairs.

\subsection{Data Expansion}
A primary challenge in leveraging historical logs is \textit{data sparsity}. For a given developer within a specific repository (\texttt{git\_repo}), historical experiments form a chronological sequence $\{E_1, E_2, \dots, E_n\}$. Relying exclusively on strictly adjacent experiments (i.e., $E_t \rightarrow E_{t+1}$) yields insufficient training data and often captures incomplete micro-edits rather than meaningful evolutionary steps. 
To overcome this, we propose a pairwise data expansion strategy. Instead of only extracting consecutive pairs, we generate all possible combinations by pairing any two experiments $(E_i, E_j)$ where $i < j$, forming $(prev, cur)$ training samples. This combinatorial approach transforms a sparse experimental sequence into a dense dataset. Beyond amplifying the sample size, it enables Astar to learn evolutionary trajectories across varying temporal distances, capturing both short-term tweaks and long-term algorithmic leaps.

\subsection{Data Denoising}
Beyond data sparsity, historical records suffer from severe \textit{noise}. To capture meaningful model evolution, we extract and process evolution-driven code differences rather than the full codebases. This eliminates unchanged boilerplate and forces Astar to focus on actual algorithmic updates. However, raw deltas remain noisy: they frequently mix core algorithmic changes with trivial engineering configurations, and many experiments entirely lack explicit evolutionary intent. Thus, we implement a two-stage denoising pipeline comprising rule-based Execution Logic Filtering and LLM-based Evolution Intent Filtering.

\subsubsection{Execution Logic Filtering}
This stage aims to isolate modifications that genuinely alter the algorithmic behavior. We achieve this through a sequence of codebase-level cleaning followed by delta-level filtering.

\paragraph{Reachability Analysis.} 
We begin by processing the individual $prev$ and $cur$ codebases independently. To ensure the extracted modifications are actually invoked during the model's lifecycle, we construct a call-graph for each codebase. Any code residing in uncalled functions or unreachable branches is identified as dead code and discarded, establishing a strictly execution-relevant foundation.

\paragraph{Syntax Normalization.} 
Continuing at the codebase level, we parse the remaining files into Abstract Syntax Trees (ASTs) to eliminate syntax-level noise that does not affect execution. This step automatically removes trivial components, such as debugging statements (e.g., \texttt{print}, \texttt{assert}) and comments, while normalizing non-functional variations like formatting adjustments and \texttt{import} sequence reordering.

\paragraph{Configuration Whitelisting.} 
After purifying the individual codebases, we employ standard differencing algorithms to compute the pairwise code differences between them. To distinguish between environmental setups and algorithmic hyperparameters within these extracted changes, we filter the modifications against a predefined parameter whitelist. Changes to engineering variables (e.g., \texttt{output\_dir}, \texttt{gpu\_count}, \texttt{job\_name}) are discarded, while core algorithmic parameters (e.g., \texttt{learning\_rate}, \texttt{optimizer}, \texttt{model\_name}) are preserved, yielding the final purified code delta.

\subsubsection{Evolution Intent Filtering}
Even after obtaining the purified code modifications, certain experimental pairs may still lack a purposeful model evolution intent. To address this, we leverage Large Language Models (LLMs) to map the code changes into explicit evolutionary semantics. Modifications that fail to map to valid evolution intents are regarded as noise and discarded, ensuring that heterogeneous code updates converge into a unified intent space.

\paragraph{Taxonomy Alignment via Hierarchical Hints.} 
We prompt the LLM to classify the purified modifications into a predefined three-level taxonomy tree (\textit{L1 Main Direction} $\rightarrow$ \textit{L2 Target Module} $\rightarrow$ \textit{L3 Specific Action}), forming structured \textit{Hierarchical Hints}. These hints effectively filter out irrelevant changes while providing Astar with dense, multi-granular supervision signals during training, and serving as structured priors to guide exploration during inference.

\paragraph{Fine-Grained Elaboration via Diff Insight.} 
Complementing the structured taxonomy, we task the LLM with generating a \textit{Diff Insight}, a concise textual explanation detailing the exact code changes. This insight captures nuanced algorithmic tweaks that the predefined taxonomy might miss, enriching the dataset with a fine-grained semantic description of the evolution intent.

\subsection{Context Construction}
To predict the optimal evolution direction, Astar must understand the system's state prior to modification. For each $(prev, cur)$ pair, we construct a comprehensive system context comprising \textit{Data Features}, which provide structured statistics of the experimental dataset (e.g., business domain, sample volume, feature dimensions) as a quantitative baseline; and a \textit{Base Insight}, an LLM-generated natural language overview of the \textit{prev} codebase summarizing the existing model architecture, core modules, and training strategies.

By pairing this state context with the denoised evolutionary signals, we formulate the final training corpus. Each instance structurally maps the initial system state to the intended evolutionary action in the format shown in Figure~\ref{fig:data_format}.
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/data_format.pdf}
    \caption{The format of the data.}
    \label{fig:data_format}
\end{figure}
